InfoSync: Information Synchronization across Multilingual Semi-structured Tables

Information Synchronization of semi-structured data across languages is challenging. For instance, Wikipedia tables in one language should be synchronized across languages. To address this problem, we introduce a new dataset InfoSyncC and a two-step method for tabular synchronization. InfoSync contains 100K entity-centric tables (Wikipedia Infoboxes) across 14 languages, of which a subset (3.5K pairs) are manually annotated. The proposed method includes 1) Information Alignment to map rows and 2) Information Update for updating missing/outdated information for aligned tables across multilingual tables. When evaluated on InfoSync, information alignment achieves an F1 score of 87.91 (en <-> non-en). To evaluate information updation, we perform human-assisted Wikipedia edits on Infoboxes for 603 table pairs. Our approach obtains an acceptance rate of 77.28% on Wikipedia, showing the effectiveness of the proposed method.

==> 07-discussion.tex <==
\section{Discussion and Future Work} 
\label{sec:discussion}

\textbf{What did we learn?} Information synchronization is a common issue for Wikipedia Infoboxes across languages. Our proposed approach is effective for both aligning and updating.
% From the analysis of tabular information mismatched (\S\ref{ssec:tablular_information_mismatched}), we show that Wikipedia Infobox are omitted in many languages. 
% This Infobox absence varies unevenly among languages and categories. In addition, even if most language variants of the Infoboxes are present, they may include obsolete or missing entries.

% We discovered that our proposed table alignment algorithm (\S\ref{ssec:method_alignment}), is effective on Infobox alignments. Most importantly, our suggested approach outperforms the prior alignment baselines. This indicates that our module-based strategy with successive constraint relaxation is better at aligning information. Ablation studies show that all modules are crucial for alignment, some more than others. We verified that our proposed rule-based updating method (\S\ref{ssec:method_updation}) is effective for editing Infobox. Thus, our proposed rules are quite general and cover different categories. Furthermore, the human-assisted updates on Wikipedia's Infobox also received a high approval score. Overall, our proposed method works well for table synchronization across languages.



%Mostly on Updation (NLP/ML Automatic Deep Learning rather Rule Based) \\
%Pair-wise alignment for now, but we want to use multiple languages round robin distributed and English-centric (central server system, message passing) reference language for multiple table alignments in one go.

% \begin{itemize}
% % \item Why Wikipedia? Why Infoboxes? Why tables? Why translation?
% % \item All Challenges not addressed or addressed?
% % \item why only wikipedia updates as future work?
% % \item Why Two step procedure for Information synchronization ?
% \end{itemize}

==> wikipedia_update.tex <==
\subsection{Human update on Wikipedia InfoBox}\label{ssec:live_updates}
\begin{itemize}
    \item Performance of our Updation Algorithm 
    \item Results (Acceptance/Rejections) from Updation
\end{itemize}
